SCUBA: Salesforce Computer Use Benchmark

We introduce SCUBA, a benchmark designed to evaluate computer-use agents on customer relationship management (CRM) workflows within the Salesforce platform. SCUBA contains 300 task instances derived from real user interviews, spanning three primary personas, platform administrators, sales representatives, and service agents. The tasks test a range of enterprise-critical abilities, including Enterprise Software UI navigation, data manipulation, workflow automation, information retrieval, and troubleshooting. To ensure realism, SCUBA operates in Salesforce sandbox environments with support for parallel execution and fine-grained evaluation metrics to capture milestone progress. We benchmark a diverse set of agents under both zero-shot and demonstration-augmented settings. We observed huge performance gaps in different agent design paradigms and gaps between the open-source model and the closed-source model. In the zero-shot setting, open-source model powered computer-use agents that have strong performance on related benchmarks like OSWorld only have less than 5\% success rate on SCUBA, while methods built on closed-source models can still have up to 39% task success rate. In the demonstration-augmented settings, task success rates can be improved to 50\% while simultaneously reducing time and costs by 13% and 16%, respectively. These findings highlight both the challenges of enterprise tasks automation and the promise of agentic solutions. By offering a realistic benchmark with interpretable evaluation, SCUBA aims to accelerate progress in building reliable computer-use agents for complex business software ecosystems.

==> tabs/results_no_mem.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{threeparttable}[!th]
% \small
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{@{}cccccccc@{}}
% \toprule
% Method Name             & Milestone Score $\uparrow$ & Success Rate $\uparrow$ & Time (min) $\downarrow$ & Steps $\downarrow$ & HA Ratio $\uparrow$ & Tokens (k) $\downarrow$ & Costs (\$) $\downarrow$ \\ \midrule
% \rowcolor{gray!15}\multicolumn{8}{c}{Browser-Use Agents}                                                                                       \\ \midrule
% \gpt{5}                 &                 &              &            &        &         &                   &           \\
% \osan                   &                 &              &            &        &         &                   &           \\
% \gemini{2.5-Pro}        &                 &              &            &        &         &                   &           \\
% \claudecua              &                 &              &            &        &         &                   &           \\ \midrule
% \rowcolor{gray!15}\multicolumn{8}{c}{Computer-Use Agents}                                                                                  \\ \midrule
% \uitars{1.5-7B}         & 0.10            &  2.67\%      &  6.14      &  35.43 &  ***    &   183.69          & -\tnote{*}    \\
% \opencua{7B}            & 0.05            &  0.67\%      & 20.48      &  31.21 &  ***    &   133.88          & -\tnote{*}    \\
% \oaicua                 & 0.29            &  16.0\%      & 5.80       &  31.32 &  0.87   &   193.83          & 0.59          \\
% \claudecua (computer)   & 0.48            &  27.0\%      & 8.02       &  35.24 &  0.75   &   457.77          & 1.44          \\ 
% \agents{2.5}(w/\gpt{5}) & 0.58            &  39.0\%      & 25.13      &  34.23 &  0.83   &   597.92          & 1.16\tnote{**} \\ \bottomrule
% \end{tabular}
% }
% \caption{Performances of various agents on the \crmbench{}. All metrics are averaged accross all instances. $\uparrow$ next to each column name represents the larger value, the better and vice-versa for $\downarrow$. }%Milestone score is normalized into [0,1]. Sucees rate is between [0,1]. Time is counted in minutes.  }
% \begin{tablenotes}
% \item[*] We do not report the inference prices for the self-hosted models.
% \item[**] This does not include the costs of serving \uitars{1.5-7B} models as the grounder used in \agents{2.5}.
% \item[***] To make HA Ratio reliable, we require the method should be successful at least 30 tasks.
% \end{tablenotes}
% \end{threeparttable}



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{threeparttable}[!th]
\small
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}ccccccc@{}}
\toprule
Method Name             & Milestone Score $\uparrow$ & Success Rate $\uparrow$ & Time (min) $\downarrow$ & Steps $\downarrow$ & Tokens (k) $\downarrow$ & Costs (\$) $\downarrow$ \\ \midrule
\rowcolor{gray!15}\multicolumn{7}{c}{Browser-Use Agents}                                                                                       \\ \midrule
\gpt{5}                 &                 &              &            &        &                     &           \\
\osan                   &                 &              &            &        &                     &           \\
\gemini{2.5-Pro}        &                 &              &            &        &                     &           \\
\claudecua              &                 &              &            &        &                     &           \\ \midrule
\rowcolor{gray!15}\multicolumn{7}{c}{Computer-Use Agents}                                                                                  \\ \midrule
\uitars{1.5-7B}         & 0.10            &  2.67\%      &  6.14      &  35.43 &     183.69          & -\tnote{*}    \\
\opencua{7B}            & 0.05            &  0.67\%      & 20.48      &  31.21 &     133.88          & -\tnote{*}    \\
\oaicua                 & 0.29            &  16.00\%     & 5.80       &  31.32 &     193.83          & 0.59          \\
\claudecua (computer)   & 0.48            &  27.00\%     & 8.02       &  35.24 &     457.77          & 1.44          \\ 
\agents{2.5}(w/\gpt{5}) & 0.58            &  39.00\%     & 25.13      &  34.23 &     597.92          & 1.16\tnote{**} \\ \bottomrule
\rowcolor{gray!15}\multicolumn{7}{c}{Computer-Use Agents}
\end{tabular}
}
\caption{Performances of various agents on the \crmbench{}. All metrics are averaged accross all instances. $\uparrow$ next to each column name represents the larger value, the better and vice-versa for $\downarrow$. }%Milestone score is normalized into [0,1]. Sucees rate is between [0,1]. Time is counted in minutes.  }
\begin{tablenotes}
\item[*] We do not report the inference prices for the self-hosted models.
\item[**] This does not include the costs of serving \uitars{1.5-7B} models as the grounder used in \agents{2.5}.
\end{tablenotes}
\end{threeparttable}

==> tabs/results_with_mem.tex <==
\begin{threeparttable}[!th]
\small
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}ccccccc@{}}
\toprule
Method Name             & Milestone Score $\uparrow$ & Success Rate $\uparrow$ & Time (min) $\downarrow$ & Steps $\downarrow$ & Tokens (k) $\downarrow$ & Costs (\$) $\downarrow$ \\ \midrule
\rowcolor{gray!15}\multicolumn{7}{c}{Browser-Use Agents}                                                                                       \\ \midrule
\gpt{5}                 &                 &              &            &        &                     &           \\
\osan                   &                 &              &            &        &                     &           \\
\gemini{2.5-Pro}        &                 &              &            &        &                     &           \\
\claudecua              &                 &              &            &        &                     &           \\ \midrule
\rowcolor{gray!15}\multicolumn{7}{c}{Computer-Use Agents}                                                                                  \\ \midrule
\uitars{1.5-7B}         & 0.24            &   9.16\%     &  6.52      &  37.65 &     213.07          & -\tnote{*}    \\
\opencua{7B}            & 0.12            &   5.38\%     & 18.86      &  33.57 &     159.11          & -\tnote{*}    \\
\oaicua                 & 0.50            &  28.85\%     &  5.29      &  27.29 &     171.93          & 0.52          \\
\claudecua (computer)   & 0.67            &  47.69\%     &  7.33      &  32.05 &     424.90          & 1.34          \\ 
\agents{2.5}(w/\gpt{5}) & 0.57            &  40.38\%     & 24.63      &  34.43 &     626.26          & 1.19\tnote{**} \\ \bottomrule
\end{tabular}
}
\caption{Performances of various agents on the \crmbench{}. All metrics are averaged accross all instances. $\uparrow$ next to each column name represents the larger value, the better and vice-versa for $\downarrow$. }%Milestone score is normalized into [0,1]. Sucees rate is between [0,1]. Time is counted in minutes.  }
\begin{tablenotes}
\item[*] We do not report the inference prices for the self-hosted models.
\item[**] This does not include the costs of serving \uitars{1.5-7B} models as the grounder used in \agents{2.5}.
\end{tablenotes}
\end{threeparttable}

==> tabs/tab-agent-performance.tex <==
\begin{table}[h!]
\centering
\caption{Success rate and milestone (\%) comparison across different tasks.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\hline
\multirow{2}{*}{\textbf{Agent}} & 
\multicolumn{2}{c}{\textbf{Account Mgmt}} & 
\multicolumn{2}{c}{\textbf{Product Int.}} & 
\multicolumn{2}{c}{\textbf{Product Search}} & 
\multicolumn{2}{c}{\textbf{Deal Search}} \\
\cline{2-9}
 & Success & Milestone & Success & Milestone & Success & Milestone & Success & Milestone \\
\hline
\oaicua &  &  &  &  &  &  &  &  \\
\uitars{1.5-7B} &  &  &  &  &  &  &  &  \\
\opencua{7B} &  &  &  &  &  &  &  &  \\
\agents{2.5+GPT5} &  &  &  &  &  &  &  &  \\
\claudecua  &  &  &  &  &  &  &  &  \\
\hline
\gpt{5} &  &  &  &  &  &  &  &  \\
\osan &  &  &  &  &  &  &  &  \\
\gemini{2.5-Pro} &  &  &  &  &  &  &  &  \\
\claude{4.0-Sonnet} &  &  &  &  &  &  &  &  \\
\hline
\end{tabular}%
}
\label{tab:performance}
\end{table}



